Fast-OMRA: Fast Online Motion Resolution Adaptation for Neural B-Frame Coding

Most learned B-frame codecs with hierarchical temporal prediction suffer from the domain shift issue caused by the discrepancy in the Group-of-Pictures (GOP) size used for training and test. As such, the motion estimation network may fail to predict large motion properly. One effective strategy to mitigate this domain shift issue is to downsample video frames for motion estimation. However, finding the optimal downsampling factor involves a time-consuming rate-distortion optimization process. This work introduces lightweight classifiers to determine the downsampling factor. To strike a good rate-distortion-complexity trade-off, our classifiers observe simple state signals, including only the coding and reference frames, to predict the best downsampling factor. We present two variants that adopt binary and multi-class classifiers, respectively. The binary classifier adopts the Focal Loss for training, classifying between motion estimation at high and low resolutions. Our multi-class classifier is trained with novel soft labels incorporating the knowledge of the rate-distortion costs of different downsampling factors. Both variants operate as add-on modules without the need to re-train the B-frame codec. Experimental results confirm that they achieve comparable coding performance to the brute-force search methods while greatly reducing computational complexity.

==> chapters/algorithm/Fast-OMRA_binary.tex <==
\begin{algorithm}[t]
\caption{Fast-OMRA}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Coding frame $x_{t}$, Reference frames $\hat{x}_{t \pm k}$, Temporal distance $d_{t}$
\STATE \textbf{Output:} Optimal Scale factor $S_{optimal}$
\IF{$d_{t} = 1$ }
    \STATE $S_{optimal}\leftarrow 1$
\ELSE
    \STATE $S_{pred} \leftarrow MotionClassification(x_{t}, \hat{x}_{t \pm k}, d_{t})$
    \IF{$S_{pred} = 1$ }
        \STATE $S_{optimal}\leftarrow 1$
    \ELSE
        \FOR{$S\in \left\{ 2, 4, 8\right\}$}
            \STATE $x_{t}^{(S)} = Down\left ( x_{t}, S \right )$
            \STATE $\hat{x}_{t\pm k}^{(S)} = Down\left ( \hat{x}_{t\pm k}, S \right )$
            \STATE $f_{t \to t \pm k}^{(S)}=ME\left ( x_{t}^{(S)}, \hat{x}_{t\pm k}^{(S)}  \right )$
            \STATE $x_{t \to t \pm k}^{(S)} = Warp\left ( \hat{x}_{t\pm k}^{(S)}, f_{t \to t \pm k}^{(S)} \right )$
        \ENDFOR
        \STATE $S_{optimal}\leftarrow \underset{S \in \{2, 4, 8\}}{\arg\min} \, MSE\left(Up\left( x_{t \to t \pm k}^{(S)}, S\right)\right)$
    \ENDIF
\ENDIF
\STATE \textbf{return} $S_{optimal}$
\end{algorithmic}
\label{algorithm:Fast-OMRA_binary}
\end{algorithm}

==> chapters/algorithm/OMRA-MEMC.tex <==
\begin{algorithm}[t]
\caption{OMRA-MEMC}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Coding frame $x_{t}$, Reference frames $\hat{x}_{t \pm k}$
\STATE \textbf{Output:} Optimal Scale factor $S_{optimal}$
\FOR{$S\in \left\{ 1, 2, 4, 8\right\}$}
    \STATE $x_{t}^{(S)} = Down\left ( x_{t}, S \right )$
    \STATE $\hat{x}_{t\pm k}^{(S)} = Down\left ( \hat{x}_{t\pm k}, S \right )$
    \STATE $f_{t \to t \pm k}^{(S)}=ME\left ( x_{t}^{(S)}, \hat{x}_{t\pm k}^{(S)}  \right )$
    \STATE $x_{t \to t \pm k}^{(S)} = Warp\left ( \hat{x}_{t\pm k}^{(S)}, f_{t \to t \pm k}^{(S)} \right )$
\ENDFOR
\STATE $S_{optimal}\leftarrow \underset{S \in \{1, 2, 4, 8\}}{\arg\min} \, MSE(x_{t \to t \pm k}^{(S)})$
\STATE \textbf{return} $S_{optimal}$
\end{algorithmic}
\label{algorithm:OMRA-MEMC}
\end{algorithm}

==> chapters/algorithm/OMRA-MEMC_star.tex <==
\begin{algorithm}[t]
\caption{OMRA-MEMC*}
\begin{algorithmic}[1]
\STATE \textbf{Input:} Coding frame $x_{t}$, Reference frames $\hat{x}_{t \pm k}$, Temporal distance $d_{t}$
\STATE \textbf{Output:} Optimal Scale factor $S_{optimal}$
\IF{$d_{t} = 1$ }
    \STATE $S_{optimal}\leftarrow 1$
\ELSE
    \FOR{$S\in \left\{ 1, 2, 4, 8\right\}$}
        \STATE $x_{t}^{(S)} = Down\left ( x_{t}, S \right )$
        \STATE $\hat{x}_{t\pm k}^{(S)} = Down\left ( \hat{x}_{t\pm k}, S \right )$
        \STATE $f_{t \to t \pm k}^{(S)}=ME\left ( x_{t}^{(S)}, \hat{x}_{t\pm k}^{(S)}  \right )$
        \STATE $x_{t \to t \pm k}^{(S)} = Warp\left ( \hat{x}_{t\pm k}^{(S)}, f_{t \to t \pm k}^{(S)} \right )$
    \ENDFOR
\STATE $S_{optimal}\leftarrow \underset{S \in \{1, 2, 4, 8\}}{\arg\min} \, MSE(x_{t \to t \pm k}^{(S)})$
\ENDIF
\STATE \textbf{return} $S_{optimal}$
\end{algorithmic}
\label{algorithm:OMRA-MEMC_star}
\end{algorithm}

==> chapters/figure/OMRA_vs_FastOMRA.tex <==
\begin{figure}[t]
    \centering
    \centerline{\includegraphics[width=0.5\textwidth]{figures/OMRA_vs_FastOMRA.png}}
    \caption{OMRA (a) versus Fast-OMRA (b).}
    \label{fig:OMRA_vs_FastOMRA}
\end{figure}

==> chapters/figure/complexity.tex <==
\begin{figure}[t]
    \centering
    \centerline{\includegraphics[width=0.5\textwidth]{figures/complexity.png}}
    \caption{Complexity comparison.}
    \label{fig:complexity}
\end{figure}

==> chapters/figure/data_distribution.tex <==
\begin{figure}[t]
    \centering
    \centerline{\includegraphics[width=0.4\textwidth]{figures/data_distribution.png}}
    \caption{Training data distribution.}
    \label{fig:data_distribution}
\end{figure}

==> chapters/figure/model_design.tex <==
\begin{figure}[tb]
    \centering
    \centerline{\includegraphics[width=0.5\textwidth]{figures/model_architecture.png}}
    \caption{Architecture of the Motion Classification network}
    \label{fig:model_architecture}
\end{figure}

==> chapters/figure/overrall_bframe_codec.tex <==
\begin{figure}[tb]
    \centering
    \centerline{\includegraphics[width=0.5\textwidth]{figures/Overall_architecture.png}}
    \caption{Architecture of our proposed method}
    \label{fig:overall}
\end{figure}

==> chapters/table/5_TemporalLayer.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{\justifying Compression performance and complexity when applying proposed method in 4 and 5 temporal layers}
\centering
\small

\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{4 TL} & \multicolumn{2}{c}{5 TL} \\
                         & BD-rate     & MAC        & BD-rate     & MAC        \\ \hline
HEVC-B                   & -7.1        & 1892.9     & -6.1        & 1733.1     \\
UVG                      & -16.4       & 1862.9     & -15.6       & 1639.8     \\
MCL                      & -9.92       & 1884.8     & -13.3       & 1687.9     \\ \hline
\end{tabular}
\label{tab:5_TL}
\end{table}

==> chapters/table/OMRA_MEMC.tex <==
\begin{table*}[t]
\caption{\justifying Comparison in terms of compression performance and computation complexity between OMRA, OMRA-MEMC and OMRA-MEMC*.}
\center
\normalsize
\begin{tabular}{ccccccc}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{BDBR}}                        & \multicolumn{3}{c}{\textbf{MAC}}                                                      \\ \cline{2-7} 
                                  & \textbf{OMRA} & \textbf{OMRA-MEMC} & \textbf{OMRA-MEMC*} & \textbf{OMRA}         & \textbf{OMRA-MEMC}            & \textbf{OMRA-MEMC*}           \\ \hline
HEVC-B                            & -10.1         & -8.7              & -8.7               & \multirow{3}{*}{5.97  M/pixel} & \multirow{3}{*}{2.24 M/pixel} & \multirow{3}{*}{2.13 M/pixel} \\
UVG                               & -16.8        & -15.4             & -15.4              &                       &                               &                               \\
MCL                               & -15.1        & -12.2              & -9.2               &                       &                               &                               \\ \hline
\end{tabular}
\label{tab:OMRA_MEMC}
\end{table*}

==> chapters/table/full_layer.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{\justifying Compression performance and complexity with 4 Temporal Layer and 5 Temporal Layer.}
\small
\center
\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{4 TL} & \multicolumn{2}{c}{5 TL} \\
                         & MAC         & BD-rate    & MAC         & BD-rate    \\ \hline
HEVC-B                   & 1972.53     & -4.72      & 1884.03     & -3.93      \\
UVG                      & 1865.79     & -13.26     & 1673.32    & -11.76     \\
MCL-JCV                  & 1863.93     & -7.68      & 1714.20    & -9.62      \\ \hline
\end{tabular}
\label{tab:full_layer}
\end{table}
